Progressive Attention Networks for Visual Attribute Prediction

We propose a novel attention model that can accurately attends to target objects of various scales and shapes in images. The model is trained to gradually suppress irrelevant regions in an input image via a progressive attentive process over multiple layers of a convolutional neural network. The attentive process in each layer determines whether to pass or block features at certain spatial locations for use in the subsequent layers. The proposed progressive attention mechanism works well especially when combined with hard attention. We further employ local contexts to incorporate neighborhood features of each location and estimate a better attention probability map. The experiments on synthetic and real datasets show that the proposed attention networks outperform traditional attention methods in visual attribute prediction tasks.

==> BMVC 2018 Camera Ready/sections/abstract.tex <==
% !TEX root = ../main.tex

\begin{abstract}
We propose a novel attention model that can accurately attends to target objects of various scales and shapes in images.
The model is trained to gradually suppress irrelevant regions in an input image via a progressive attentive process over multiple layers of a convolutional neural network.
The attentive process in each layer determines whether to pass or block features at certain spatial locations for use in the subsequent layers.
The proposed progressive attention mechanism works well especially when combined with hard attention.
%We further employ local contexts to estimate attention probability at each location since it is difficult to infer accurate attention by observing a feature vector from a single location only.
We further employ local contexts to incorporate neighborhood features of each location and estimate a better attention probability map.
The experiments on synthetic and real datasets show that the proposed attention networks outperform traditional attention methods in visual attribute prediction tasks.
\end{abstract}

==> BMVC 2018 Camera Ready/sections/conclusion.tex <==
% !TEX root = ../main.tex

\vspace{-0.3cm}
\section{Conclusion}
\vspace{-0.1cm}
\label{conclusion}
We proposed a novel attention network, which progressively attends to regions of interest through multiple layers in a CNN.
%{\color{red}\st{Since our attention model is applied to multiple layers in a recursive manner, it is conceptually more effective to identify regions of interest with variable sizes and shapes.}}
As the model is recursively applied to multiple layers of a CNN with an inherent feature hierarchy, it  accurately predicts regions of interest with variable sizes and shapes.
%Since our attention model is applied to multiple layers in a recursive manner, it is conceptually more effective to identify regions of interest with variable sizes and shapes.
%While a feature in an attended feature map is used for building next feature map through next layers, a feature itself cannot give enough information for its usefulness. 
%This limitation makes the network unstable to train. 
We also incorporate local contexts into our attention network for more robust estimation.
%{\color{red}\st{The proposed network can be trained end-to-end since every operation within the network is differentiable as in the soft attention, and demonstrates significant performance improvement over existing attention methods.}}
%\brk{The proposed network is trained end-to-end with a standard error backpropagation.
%We tested the model on both synthetic and real datasets, and demonstrated substantial performance improvement over existing methods.
%}
%\hsseo{
While progressive attention networks can be implemented with either soft or hard attention, we demonstrated that both versions of the model substantially outperform existing methods on both synthetic and real datasets.
%}


==> BMVC 2018 Camera Ready/sections/experiments.tex <==
% !TEX root = ../main.tex

\vspace{-0.3cm}
\section{Experiments}
\vspace{-0.2cm}
\label{exp}
This section discusses experimental results on two datasets.
Note that our experiments focus on the tasks directly related to visual attention to minimize any artifacts caused by irrelevant components.
The codes are available at \href{https://github.com/hworang77/PAN}{https://github.com/hworang77/PAN}.



\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figures/ex_dataset/1_00001.png}
\vspace{-0.1cm}
\subcaption{MREF}
\label{fig:MREF}
\end{subfigure}~~~~~~
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figures/ex_dataset/2_00015.png}
\vspace{-0.1cm}
\subcaption{MDIST}
\label{fig:MDIST}
\end{subfigure}~~~~~~
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\linewidth]{figures/ex_dataset/3_00003.png}
\vspace{-0.1cm}
\subcaption{MBG}
\label{fig:MBG}
\end{subfigure}
\label{fig:ex_dataset}
\caption{Example of the MREF datasets.}
\vspace{-0.5cm}
\end{figure}

\vspace{-0.3cm}
\subsection{MNIST Reference}
\vspace{-0.1cm}
\paragraph{Datasets}
We conduct experiments on synthetic datasets created from MNIST~\cite{MNIST}.
The first synthetic dataset is referred to as MNIST Reference (MREF; Figure~\ref{fig:MREF}), where each training example is a triple of an image, a  query number, and its color label.
The task on this dataset is to predict the color of the number given by a query.
Five to nine distinct MNIST digits with different colors out of $\{\text{green},\text{yellow},\text{white},\text{red},\text{blue}\}$ and scales in $[0.5, 3.0]$ are randomly sampled and located within a $100\times100$ empty image with black background.
%While the image of a triple contains 5 to 9 distinct numbers with different colors in $100\times100$ space, the target task is to predict the color of the target number that is specified by the query number.
%To see models' capabilities of attending on scale variant regions, MNIST images are scaled by a factor uniformly sampled from 0.4 to 1.5.
%The color of each number is also uniformly sampled from five different colors $\{\text{green},\text{yellow},\text{white},\text{red},\text{blue}\}$.
When coloring numbers, Gaussian noise is added to the reference color value.
%
To simulate more realistic situations, we made two variants of MREF by adding distractors (MDIST; Figure~\ref{fig:MDIST}) or replacing background with natural images (MBG; Figure~\ref{fig:MBG}).
Distractors in MDIST are constructed with randomly cropped $5\times5$ patches of MNIST images whereas backgrounds of MBG are filled with natural scene images randomly chosen from the SUN Database~\cite{SUN}.
The training, validation and test sets contain 30K, 10K and 10K images, respectively.

\begin{figure}[t]
\centering
\begin{subfigure}{0.5\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{./figures/net_architecture.pdf}
\vspace{-0.1cm}
\subcaption{Network architectures of models on MREF. Arrows represents direct connection to next layer without attention.}
\label{fig:net_architecture}
\vspace{-0.2cm}
\end{subfigure}~~~~~~~
\begin{subfigure}{0.4\textwidth}
\centering
\includegraphics[width=0.9\textwidth]{./figures/att_architecture.pdf}
\vspace{-0.1cm}
\subcaption{Architecture of attention function $g^l_{\mathrm{att}}(\cdot)$.  Local contexts $\mathcal{F}^l_{i, j}$ are used only in PAN[*]+CTX.}
\label{fig:att_architecture}
\end{subfigure}
\vspace{0.3cm}
\caption{
Detailed illustration of network architectures on MNIST Reference experiments. 
}
\label{fig:network_details}
\end{figure}




\paragraph{Experimental setting}

We implement two variants of the proposed network with soft and hard attention at its final layer, denoted by PAN[S] and PAN[H], respectively.
Each of them is implemented with and without the local context observation; the networks with local context observation are denoted by `+CTX' in our results. 
%In addition, three different baselines, soft attention network (SAN), hard attention network (HAN)~\citep{showAtt} and spatial transformer network (STN)~\citep{STN}, are used for comparisons.
In addition, soft attention network (SAN), hard attention network (HAN)~\cite{showAtt}, and two variants of spatial transformer network (STN-S and STN-M)~\cite{STN} are used as baseline models for comparisons.
%
While STN-S is the model with a single transformer layer, STN-M contains multiple transformer layers in the network.
%The implementations of SAN and STN follow  the descriptions in \citep{showAtt} and \citep{STN}, respectively, while HAN is trained by optimizing the marginal log-likelihood loss since it should be more accurate and feasible due to small search space in our task. 
We reimplemented SAN and STNs following the descriptions in \cite{showAtt} and \cite{STN}, respectively, and trained HAN by optimizing the marginal log-likelihood.
%as for our model with hard attention.
%The architecture of image encoding network in SAN and HAN and localization network in STN are all identical.
The architecture of image encoding networks in SAN and HAN, and localization networks in STNs are all identical for fair comparisons.
The CNN in the proposed network also has the same architecture except for the additional layers for progressive attention.
The CNN is composed of four stacks of $3\times3$ convolutions with 32 channels (stride 1) followed by a $2\times2$ max pooling layer (stride 2) as illustrated in Figure~\ref{fig:net_architecture}.
%
%
We used a single fc layer for attribute classifier because the task requires simple color prediction. 
The attention functions $g^l_{\mathrm{att}}(\cdot)$ for all models are given by multi-layer perceptrons with two layers (Figure~\ref{fig:att_architecture}).
%
The function takes the concatenation of a query vector $q$ and a feature vector $f^l_{i,j}$, and outputs an attention score $s^l_{i,j}$, where the query vector $q$ is a one-hot vector representing a target object.
%{\color{red}the concatenation of a query $q$, which is a one-hot vector representing a target object and a feature vector $f^l_{i,j}$, and outputs an attention score $s^l_{i,j}$.}
%In PAN[*]-CTX, the attention functions of $\mathrm{att1}$, $\mathrm{att2}$ and $\mathrm{att3}$ additionally take the local context $\mathcal{F}^l_{i, j}$ containing the adjacent features with $\delta=1$.
In the proposed models, the intermediate attention functions additionally take local context $\mathcal{F}^l_{i, j}$ containing spatially adjacent features with $\delta=1$.
Every model is trained end-to-end from scratch by RMSprop until the models show no improvement for 50 epochs.
We exponentially decay the initial learning rate by 0.9 at every 30 epoch after the 50th epoch, and grid-search the best initial learning rate for each model in [0.001, 0.005].


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.4\linewidth]{figures/net_architecture.pdf}
% \caption{Architectures of models on MREF. Arrows represent direct connections to next layer without attention.}
% \label{fig:net_architecture}
% \end{figure}
%
% \begin{figure}[t]
% \centering
% \includegraphics[width=0.7\linewidth]{figures/att_architecture.pdf}
% \vspace{-0.2cm}
% \caption{Architecture of attention function $g^l_{\mathrm{att}}(\cdot)$.  Local contexts $\mathcal{F}^l_{i, j}$ are used only in PAN-CTX.}
% \label{fig:att_architecture}
% \vspace{-0.2cm}
% \end{figure}

\begin{table}[t]
\centering
\caption{Results on MREF datasets: (left) color prediction accuracy [\%] and true-positive ratio [\%]. (right) accuracy [\%] with different scales on MBG test subset.}
\label{tab:MNIST_acc}
\vspace{0.3cm}
\scalebox{0.7}{
\begin{tabular}{
@{}C{2.2cm}@{}|@{}C{1.1cm}@{}@{}C{1.1cm}@{}|@{}C{1.1cm}@{}@{}C{1.1cm}@{}|@{}C{1.1cm}@{}@{}C{1.1cm}@{}
}
		    & \multicolumn{2}{c|}{MREF} & \multicolumn{2}{c|}{MDIST}    & \multicolumn{2}{c}{MBG}   \\ 
            & Acc.      & TPR		    & Acc.      & TPR		        & Acc.      & TPR		    \\ \hline
Uniform     & 20.00     & 2.34		    & 20.00     & 2.35              & 20.00     & 2.39          \\ \hline
STN-S 	    & 39.10		& 0.94		    & 38.32		& 0.52              & 32.27	    & 0.74          \\
STN-M	    & 93.89		& 0.66		    & 85.09		& 0.74              & 52.25	    & 0.65          \\ \hline
SAN		    & 82.94		& 13.83		    & 75.73		& 12.82             & 53.77	    & 6.92          \\
HAN		    & 81.84		& 13.95		    & 78.49		& 13.81             & 55.84	    & 7.64          \\
PAN[S]	    & 95.92		& 44.25		    & 91.65		& 52.85             & 69.46	    & 32.07         \\
PAN[H]	    & 95.32     & 62.31         & 90.46		& 52.07             & 72.50	    & 38.32         \\
PAN[S]+CTX  & 98.51		& 60.45         & \bf96.02	& 59.60             & 81.01	    & 43.87         \\
PAN[H]+CTX  & \bf98.53	& \bf62.36      & 95.82		& \bf61.39          & \bf84.62	& \bf51.49      \\ \hline
\end{tabular}
}
%
\scalebox{0.7}{
\begin{tabular}{
@{}C{2.2cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.3cm}@{}@{}C{1.3cm}@{}
}
		    & \multicolumn{5}{c}{Scale ranges}                     \\ 
            & 0.5-1.0   & 1.0-1.5       & 1.5-2.0   & 2.0-2.5       & 2.5-3.0   \\ \hline
STN-S 	    & 31.1		& 35.3		    & 35.8		& 37.7          & 45.0	    \\
STN-M	    & 51.8		& 58.3		    & 55.3		& 58.5          & 61.7	    \\ \hline
SAN		    & 49.1		& 68.9		    & 63.6		& 61.7          & 54.6	    \\
HAN		    & 51.2		& 68.7		    & 70.8		& 64.0          & 59.5	    \\
PAN[S]	    & 67.9		& 76.6		    & 73.9		& 69.6          & 61.3	    \\
PAN[H]	    & 70.8      & 79.6          & 76.8		& 70.2          & 67.3	    \\
PAN[S]+CTX  & 79.6		& 86.8          & 85.1      & \bf81.9       & 72.1	    \\
PAN[H]+CTX  & \bf84.2	& \bf87.1       & \bf87.5	& 81.6          & \bf79.6	\\ \hline
\end{tabular}
}
\vspace{-0.1cm}
\end{table}


%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth] {figures/MREF_qualitative.pdf}
\vspace{-0.5cm}
\caption{
Qualitative results of SAN, HAN, PAN[S]+CTX and PAN[H]+CTX. 
%(a) Input images faded by attended feature map (c).
(a) Magnitude of activations in feature maps $f^l_{i,j}$ before attention; the activations are mapped to original image space by spreading activations to their receptive fields.
(b) Magnitude of activations in attended feature maps $\hat{f}^l_{i,j}$ showing the effect of attention in contrast to (a).
%(d) Magnitude of activations of the attended feature maps $\hat{f}^l_{i,j}$ in its original resolution of the feature map.
For PAN[$*$]+CTX, we only show last two attentions, which accumulate the attentions of earlier layers.
%For HAN, (b) represents attention probability because attended feature map is not available.
Every map is rescaled into $[0, 1]$ by $(x-\min)/(\max-\min)$.
}
\label{fig:MREF_qualitative}
\vspace{-0.3cm}
\end{figure*}
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%

\paragraph{Results}
Table~\ref{tab:MNIST_acc}(left) presents color prediction accuracy of all compared algorithms.
PAN[$*$] clearly outperforms other approaches with significant margins and PAN[$*$]+CTX further improves performance by exploiting local context for attention estimation.
%\hsseo{
Our progressive attention model with the hard attention process and local context achieves the best performance in most cases.
%}
%\brk{When applying hard attention process via marginalization to our progressive attention model and local context, we achieve the best performance in most cases.}
%
%
% \iffalse
% \begin{table}[t]
% \centering
% \caption{True-positive ratio [\%] on MREF datasets}
% \label{tab:MNIST_ratio}
% \vspace{-0.2cm}
% \scalebox{0.8}{
% \begin{tabular}[m]{
% @{}C{2.8cm}@{}|@{}C{2cm}@{}@{}C{2cm}@{}@{}C{2cm}@{}
% }
% 			& MREF 		& MDIST		& MBG	\\ \hline
% Uniform		& 2.34		& 2.35		& 2.39	\\ \hline
% STN-S		& 0.94		& 0.52		& 0.74	\\
% STN-M		& 0.66		& 0.74		& 0.65	\\ \hline
% SAN			& 13.61		& 12.56		& 6.73	\\
% HAN			& 13.95		& 13.81		& 7.64	\\
% PAN			& 17.39		& 13.10		& 8.62	\\
% HPAN		& 12.05		& 11.83		& 9.83	\\
% PAN-CTX		& 22.59		& 22.80		& 11.01	\\
% HPAN-CTX	& \bf24.19	& \bf23.92	& \bf19.16	\\
% \end{tabular}
% }
% \vspace{-0.4cm}
% \end{table}
% \fi
%
Note that the attention capability of the baseline models is restricted to either rhombic or coarsely shaped regions.
In contrast, the proposed networks predict attention maps with arbitrary shapes by capturing spatial support of target area better.

We also present the attention quality of the models using true-positive ratio (TPR) in Table~\ref{tab:MNIST_acc}(left).
TPR measures how strong attention is given to proper location by computing the ratio of the aggregated attention probability within the desired area (\ie ground-truth segmentation) to the attention probability in the whole image.
To calculate TPR of STN baselines, we assigned the uniform attention probabilities to the attended rhombic regions.
%PR measures the overlaps between ground-truth segmentations and binarized segmentation predictions constructed with different thresholds (Figure~\ref{fig:PR-curve}).
The models with progressive attention give the best results with significant margins compared to all the other methods.
%Note that two variants of the proposed model give the best results with significant margin compared to all the other methods.
These results suggest that progressive attention constructs more accurate shapes of attended regions than all other attention models.
Integrating hard attention and local context further improves overall performance in most cases.
%We also observe that hard attention shows additional strength in predicting the correct attention.

To evaluate scale sensitivity, we divide test sets into five subsets based on target object scales with uniform intervals and computed accuracies of the models.
%as shown in Figure~\ref{fig:MREF_scale}. 
%The performances of SAN and HAN degrade with wild scale changes and they especially fails to predict the correct answer of small objects.
%The results from MDIST are presented in Figure~\ref{fig:MREF_scale}, where SAN and HAN tend to predict the correct answers only in a scale range between 1.0 and 2.0, while their performance is degraded significantly with wild scale changes.
%STN-M becomes vulnerable to scale variations in more realistic settings.
In Table~\ref{tab:MNIST_acc}(right), the results on MBG show that the models with progressive attention are robust to scale variations due to their multi-scale attention mechanism especially when the hard attention and local contexts are incorporated.
The tendencies on MREF and MDIST are also similar.

% {\color{red}
% We also observe that hard attention generally shows better performances in accuracy and TPR compared to soft attention for attribute prediction especially in realistic settings.
% This is observed not only from the baseline comparisons but also from the comparisons among the proposed models.
% hard attention vs. soft attention
% }

An important observation regarding to STNs is that these models actually do not attend to target objects.
Instead, STNs generate almost identical transformation regardless of input images and pass the filtering process to next layers.
As the results, the transformed images are padded ones containing the entire original image with different affine transformations. 
Consequently, these models show very low TPRs, even lower than the uniform attention.


\iffalse
\brk{
An important observation regarding to the attention quality of STNs is that these models actually do not attend to the target object.
Instead, STN-M generates almost identical transformations for each query regardless of given images.
Then, the CNN learns the representations to highlight target regions for each query using the transformed images.
In other words, STN-M establishes a completely different encoding path to solve the reference problems.
The behavior of STN-S is a bit different, but the patterns of problem solving are similar.
%Instead, STNs generate almost identical transformations for each query regardless of the given image and manipulate the transformations to avoid non-target objects from being captured by the next convolution layers.
Since the transformer layers do not recognize the location of the object and pass the filtering process to the next convolution layers, the transformed images are padded images containing the entire original image in different affine transformations. 
In consequence, these models show very low TPRs, even lower than the uniform attention.
%See the supplementary document for some qualitative results of STN transformations.
}
\fi




% \begin{table}[t]
% \centering
% \caption{Color prediction accuracy [\%] and true-positive ratio [\%] on MREF datasets.}
% \label{tab:MNIST_acc}
% \vspace{0.2cm}
% \scalebox{0.7}{
% \begin{tabular}[m]{
% @{}C{2.3cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}|@{}C{1.3cm}@{}@{}C{1.3cm}@{}
% }
% 		    & \multicolumn{2}{c|}{MREF} & \multicolumn{2}{c|}{MDIST}    & \multicolumn{2}{c}{MBG}   \\ 
%             & Acc.      & TPR		    & Acc.      & TPR		        & Acc.      & TPR		    \\ \hline
% Uniform     & 20.00     & 2.34		    & 20.00     & 2.35              & 20.00     & 2.39          \\ \hline
% STN-S 	    & 39.10		& 0.94		    & 38.32		& 0.52              & 32.27	    & 0.74          \\
% STN-M	    & 93.89		& 0.66		    & 85.09		& 0.74              & 52.25	    & 0.65          \\ \hline
% SAN		    & 82.94		& 13.83		    & 75.73		& 12.82             & 53.77	    & 6.92          \\
% HAN		    & 81.84		& 13.95		    & 78.49		& 13.81             & 55.84	    & 7.64          \\
% PAN[S]	    & 95.92		& 44.25		    & 91.65		& 52.85             & 69.46	    & 32.07         \\
% PAN[H]	    & 95.32     & 62.31         & 90.46		& 52.07             & 72.50	    & 38.32         \\
% PAN[S]+CTX  & 98.51		& 60.45         & \bf96.02	& 59.60             & 81.01	    & 43.87         \\
% PAN[H]+CTX  & \bf98.53	& \bf62.36      & 95.82		& \bf61.39          & \bf84.62	& \bf51.49      \\ \hline
% \end{tabular}
% }
% \end{table}








% \begin{figure}[t]
% \centering
% \begin{subfigure}{0.53\textwidth}
% \centering
% \scalebox{0.7}{
% \begin{tabular}{
% @{}C{2.2cm}@{}|@{}C{1.2cm}@{}@{}C{1.2cm}@{}|@{}C{1.2cm}@{}@{}C{1.2cm}@{}|@{}C{1.2cm}@{}@{}C{1.2cm}@{}
% }
% 		    & \multicolumn{2}{c|}{MREF} & \multicolumn{2}{c|}{MDIST}    & \multicolumn{2}{c}{MBG}   \\ 
%             & Acc.      & TPR		    & Acc.      & TPR		        & Acc.      & TPR		    \\ \hline
% Uniform     & 20.00     & 2.34		    & 20.00     & 2.35              & 20.00     & 2.39          \\ \hline
% STN-S 	    & 39.10		& 0.94		    & 38.32		& 0.52              & 32.27	    & 0.74          \\
% STN-M	    & 93.89		& 0.66		    & 85.09		& 0.74              & 52.25	    & 0.65          \\ \hline
% SAN		    & 82.94		& 13.83		    & 75.73		& 12.82             & 53.77	    & 6.92          \\
% HAN		    & 81.84		& 13.95		    & 78.49		& 13.81             & 55.84	    & 7.64          \\
% PAN[S]	    & 95.92		& 44.25		    & 91.65		& 52.85             & 69.46	    & 32.07         \\
% PAN[H]	    & 95.32     & 62.31         & 90.46		& 52.07             & 72.50	    & 38.32         \\
% PAN[S]+CTX  & 98.51		& 60.45         & \bf96.02	& 59.60             & 81.01	    & 43.87         \\
% PAN[H]+CTX  & \bf98.53	& \bf62.36      & 95.82		& \bf61.39          & \bf84.62	& \bf51.49      \\ \hline
% \end{tabular}
% }
% %\subcaption{}
% %\label{tab:MNIST_acc}
% \end{subfigure}
% \begin{subfigure}{0.45\textwidth}
% \centering
% \includegraphics[width=1\linewidth] {figures/MREF_scale/scale_bg.pdf}
% \vspace{-0.43cm}
% %\subcaption{}
% %\subcaption{Attribute prediction accuracies of different models on test subsets with different scales in MBG.}
% %\label{fig:MREF_scale}
% \end{subfigure}
% \caption{Results on MREF datasets: (left) color prediction accuracy [\%] and true-positive ratio [\%]. (right) accuracy with different scales on MBG test subset.}
% \label{tab:MNIST_acc}
% \vspace{-0.3cm}
% \end{figure}










\iffalse
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering
\begin{subfigure}[b]{1.0\textwidth}
\centering
\includegraphics[width=0.32\textwidth] {figures/MREF_scale/scale_clean.pdf}
\includegraphics[width=0.32\textwidth] {figures/MREF_scale/scale_cluttered.pdf}
\includegraphics[width=0.32\textwidth] {figures/MREF_scale/scale_bg.pdf}
\vspace{-0.3cm}
\subcaption{Attribute prediction accuracies of different models on the test subsets in different scales.}
\label{fig:MREF_scale}
\end{subfigure}
\centering
\begin{subfigure}[b]{1\textwidth}
\centering
\includegraphics[width=0.32\textwidth] {figures/PR_curve/pr-curve_clean.pdf}
\includegraphics[width=0.32\textwidth] {figures/PR_curve/pr-curve_cluttered.pdf}
\includegraphics[width=0.32\textwidth] {figures/PR_curve/pr-curve_bg.pdf}
\vspace{-0.3cm}
\subcaption{The precision-recall curves of object segmentation with attention probability.}
\label{fig:PR-curve}
\end{subfigure}
\vspace{-0.5cm}
\caption{Analysis of algorithms on MREF (left), MDIST (middle), and MBG (right).}
\vspace{-0.25cm}
\end{figure*}
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\fi

Figure~\ref{fig:MREF_qualitative} illustrates qualitative results of the two proposed methods and two baselines on MBG dataset. 
Our models yield accurate attended regions by gradually augmenting attention and suppressing irrelevant regions in the image.
We observe that the proposed models maintain high attention resolution through the progressive attention process.
In contrast, the baseline models attend to target regions only once at the top layer resulting in coarse attention. % in size and shape.
%More qualitative results are presented in the supplementary document.
%explain the means of drawing the qualitative results




\subsection{Attribute prediction on Visual Genome}
\vspace{-0.1cm}
\paragraph{Dataset}
Visual Genome (VG)~\cite{VisGen} is an image dataset containing several types of annotations: question/answer pairs, image captions, objects, object attributes and object relationship. 
We formulate object attribute prediction as a multi-label classification task with reference.
Given an input image and a query (\ie an object category), we predict binary attributes of individual objects specified by the query.
We used 827 object classes and 749 attribute classes that appear more than 100 times.
A total of 86,674 images with 667,882 object attribute labels are used for our experiment, and they are split into training, validation and test sets, which contain 43,337, 8,667 and 34,670 images, respectively.
The task is challenging because appearances and semantics of objects largely vary.
%The dataset is challenging for several reasons. 
%First, the annotations are noisy and incomplete because the object and attribute annotations are only extracted from the annotated captions by crowdsourcing. 
%There are many missing objects and attributes not mentioned in any captions.
%Second, scales of objects largely vary and the attributes may be associated with very small objects.
%Third, the attribute labels for objects are highly skewed. 
%For each object, only about 1.2 attributes out of 274 are annotated as positive on average while all others are negative.
%Finally, some of the annotated objects and attributes are even invisible or indistinguishable using the object query (\eg {\it{air}}, {\it{it}} and {\it{something}}).

\begin{table}[t]
\centering
\caption{Weighted mAP of the attribute prediction and TPR of attentions measured with ground-truth bounding boxes on VG dataset (left). TPR of attentions measured with ground-truth segmentations in VOC 2007 (right).} 
\vspace{0.2cm}
\label{tab:VisGen_result}
\scalebox{0.7}{
\begin{tabular}[m]{
@{}C{2.5cm}@{}|@{}C{1.5cm}@{}@{}C{1.5cm}@{}|@{}C{1.5cm}@{}@{}C{1.5cm}@{}
}
			& \multicolumn{2}{c|}{attention only} 			& \multicolumn{2}{c}{w/ prior}  \\ 
			& mAP 		& TPR		& mAP		& TPR		\\ \hline
STN-S		& 28.87		& 11.59		& 30.50		& 7.78		\\
STN-M		& 29.12		& 1.99		& 31.17		& 2.28		\\ \hline
SAN			& 27.62		& 15.01		& 31.84		& 17.65		\\
HAN			& 27.72		& 17.24		& 31.93		& 19.70		\\
PAN[S]+CTX	& 29.38 	& 18.01 	& 32.50 	& 20.17 	\\
PAN[H]+CTX	& \bf{30.00}& \bf{22.23}& \bf{34.19}& \bf{24.37}\\ \hline
\end{tabular}
}~~~~~
\scalebox{0.7}{
\begin{tabular}[m]{
@{}C{2.5cm}@{}|@{}C{2.8cm}@{}
}
            & TPR (VOC 2007)    \\ \hline
SAN			& 22.01		        \\
HAN         & 24.91             \\
PAN[S]+CTX  & 27.16             \\
PAN[H]+CTX  & \bf31.79          \\ \hline
\end{tabular}
}
\vspace{-0.2cm}
\end{table}
%
\paragraph{Experimental settings and results}
%We mainly compare our algorithm with SAN and HAN since STNs could not learn a proper attention process on VG.
%The transformer layers of STNs generated padded images of different sizes and rotations to encode the query vector to fit the query-specific biases.
All networks share VGG-16 network~\cite{VGG16} pretrained on ImageNet~\cite{ImageNet} and is further fine-tuned for attribute prediction.
For SAN and HAN, an attention layer is attached to the last pooling layer of VGG-16 while PAN[S]+CTX and PAN[H]+CTX stack an additional attention layer with local contexts $\mathcal{F}^l_{i, j}$ with $\delta=2$ on top of the last three pooling layers in VGG-16.
We skip the first two pooling layers ($\mathrm{pool1}$ and $\mathrm{pool2}$) for placing attention because the features in those layers are not discriminative enough to filter out. % postponing the suppression by predicting $\alpha^l_{i,j}=1$ for all $i$ and $j$.
We also test the models with object class conditional prior.
For the purpose, the final attended feature is fused with the query once more using a fully connected layer, which allows the network to reflect the conditional distribution of the attributes given the query.
We train the models by Adam with different module-wise initial learning rates and the initial learning rates are exponentially decayed by the factor of 0.9.
Refer to the supplementary document and the code for more detailed descriptions on the network architectures and experimental settings, respectively.

All models are evaluated via mean average precision (mAP) weighted by the frequencies of the attribute labels in test set, where the computation of mAP follows PASCAL VOC protocol~\cite{voc}.
Our progressive attention process with local context and hard attention mechanism consistently achieves the best weighted mAP scores in both experimental settings as shown in Table~\ref{tab:VisGen_result}(left). %but the gain reduces with object class conditional prior.
Table~\ref{tab:VisGen_result}(left) also presents TPR of each model measured with ground-truth bounding boxes due to lack of the ground-truth segmentation labels for evaluating attention qualities.
PAN[H]+CTX shows the best TPR although the computation of TPR with bounding boxes is more favorable to other methods.
%
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth] {figures/VG_qualitative.pdf}
\caption{
Visualization of example attentions of models on VG dataset.
Two variants of progressive attention models gradually attend to target objects (queried by {\it{sign}}) in fine resolution. For PAN[$*$]+CTX, we only show last two attentions, which accumulate attentions of earlier layers.
More qualitative results are presented in supplementary document.
}
\label{fig:VG_qualitative}
\vspace{-0.5cm}
\end{figure*}
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%

% \begin{table}[t]
% \centering
% \caption{Weighted mAP of the attribute prediction and TPR of attentions measured with ground-truth bounding boxes on VG dataset.} 
% \label{tab:VisGen_result}
% \vspace{-0.2cm}
% \scalebox{0.8}{
% \begin{tabular}[b]{
% @{}C{2.5cm}@{}|@{}C{1.5cm}@{}@{}C{1.5cm}@{}|@{}C{1.5cm}@{}@{}C{1.5cm}@{}
% }
% 			& \multicolumn{2}{c|}{attention only} 			& \multicolumn{2}{c}{w/ prior}				\\ 
% 			& mAP 		& TPR		& mAP		& TPR		\\ \hline
% STN-S		& 28.87		& 11.59		& 30.50		& 7.78		\\
% STN-M		& 29.12		& 1.99		& 31.17		& 2.28		\\ \hline
% SAN			& 27.62		& 15.01		& 31.84		& 17.65		\\
% HAN			& 27.72		& 17.24		& 31.93		& 19.70		\\
% PAN[S]+CTX	& 29.38 	& 18.01 	& 32.50 	& 20.17 	\\
% PAN[H]+CTX	& \bf{30.00}& \bf{22.23}& \bf{34.19}& \bf{24.37}\\ \hline
% \end{tabular}
% }
% \vspace{-0.2cm}
% \end{table}


To measure the attention quality with segmentation masks, we also measure TPRs of models on train/val set in PASCAL VOC 2007~\cite{voc2007} as shown in Table~\ref{tab:VisGen_result}(right).
We use class names as queries for images to obtain an attention map of each image and measure TPR with its corresponding object segmentation mask.
We observe that our progressive attention models outperform the baselines and become stronger when incoporated with hard attention.
% \begin{table}[t]
% \centering
% \caption{TPR of attentions measured with ground-truth segmentations in VOC 2007.} 
% \label{tab:voc_tpr}
% \vspace{-0.4cm}
% \scalebox{0.8}{
% \begin{tabular}[b]{
% @{}C{2.8cm}@{}|@{}C{1.5cm}@{}@{}C{1.5cm}@{}@{}C{2.3cm}@{}@{}C{2.3cm}@{}
% }
% 			            & SAN 		& HAN		& PAN[S]+CTX& PAN[H]+CTX\\ \hline
% TPR (VOC 2007)			& 22.01		& 24.91		& 27.16		& \bf31.79	\\ \hline
% \end{tabular}
% }
% \vspace{-0.3cm}
% \end{table}

%
STNs have trouble to attend to target objects as in MREF and show very poor TPRs.
Note that STNs show higher mAPs than the other baselines in `attention only' setting.
We believe that this is because STNs utilize object class conditional priors by encoding queries through a manipulation in the transformation process.
Figure~\ref{fig:VG_qualitative} presents qualitative results on VG dataset, which show that the progressive attention models gradually attend to target objects.
%More qualitative results are also presented in the supplementary document.


==> BMVC 2018 Camera Ready/sections/introduction.tex <==
% !TEX root = ../main.tex

\section{Introduction}
Attentive mechanisms often play important roles in modern neural networks (NNs) especially in computer vision tasks.
Many visual attention models have been introduced in the previous literature, and they have shown that attaching an attention to NNs improves the accuracy in various tasks such as image classification~\cite{STN,multiAtt,foveal}, image generation~\cite{draw}, image caption generation~\cite{showAtt} and visual question answering~\cite{askAtt,stackAtt,noh2016training}.

There are several motivations for incorporating attentive mechanisms in NNs.
%One of them is that it is analogous to the human perceptual process. % of human beings.
One of them is analogy to the human perceptual process.
The human visual system often pays attention to a region of interest instead of processing an entire scene.
Likewise, in a neural attention model, we can focus only on attended areas of the input image.
%\brk{This benefits us in terms of computational resources;}
%\hsseo{
This is beneficial in terms of computational cost; 
%}
the number of hidden units may be reduced since the hidden activations only need to encode the region with attention~\cite{recurrentAtt}. 

Another important motivation is that various high-level computer vision tasks should identify a particular region for accurate attribute prediction.
%For example, there are some tasks to require to attend one of the objects specified by an additional input.
%For example, when an input image contains multiple objects, we often require to focus on the object specified by an additional input.
Figure~\ref{fig:ref_eg} illustrates an example task to predict the color (answer) of a given input number (query).
The query specifies a particular object in the input image (`7' in this example) for answering its attribute (red).
To address this type of tasks, the network architecture should incorporate an attentive mechanism either explicitly or implicitly.

One of the most popular attention mechanisms for NNs is soft attention~\cite{showAtt}, which aggregates responses in a feature map weighted by their attention probabilities.
% (see Appendix~\ref{satt} for more details).
This process results in a single attended feature vector.
%Refer to Appendix~\ref{satt} for details of soft attention.
Since the soft attention method is fully differentiable, the entire network can be trained end-to-end using a standard backpropagation.
%However, it allocates attention probabilities to regions with a fixed size and shape as it maps from the receptive field of each location in the feature map.
However, it can only model attention to local regions with a fixed size depending on the receptive field of the layer chosen for attention.
This makes the soft attention method inappropriate for complicated cases, where objects involve significant variations in their scale and shape.



% %
% %%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
% \begin{figure*}[t]
% \centering
% \begin{subfigure}[b]{0.19\textwidth}
% \centering
% \includegraphics[width=0.8\textwidth]{figures/ref_eg/0.png}
% \subcaption{input image}
% \end{subfigure}
% \begin{subfigure}[b]{0.19\textwidth}
% \centering
% \includegraphics[width=0.8\textwidth]{figures/ref_eg/1.png}
% \subcaption{first attention}
% \end{subfigure}
% \begin{subfigure}[b]{0.19\textwidth}
% \centering
% \includegraphics[width=0.8\textwidth]{figures/ref_eg/2.png}
% \subcaption{second attention}
% \end{subfigure}
% \begin{subfigure}[b]{0.19\textwidth}
% \centering
% \includegraphics[width=0.8\textwidth]{figures/ref_eg/3.png}
% \subcaption{third attention}
% \end{subfigure}
% \begin{subfigure}[b]{0.19\textwidth}
% \centering
% \includegraphics[width=0.8\textwidth]{figures/ref_eg/4.png}
% \subcaption{final attention}
% \end{subfigure}
% \caption{
% An example reference problem (with the query 7 and the answer {\it{red}}) and intermediate attention maps using our progressive attention model. 
% It shows that attention is gradually refined through the network layers for resolving the reference problem. Distracting patterns in smaller scales are suppressed at earlier layers while those in larger scales (\eg 9) are suppressed at later layers with larger receptive fields.
% All attended images are independently rescaled for better visualization and are best-viewed in color.}
% \label{fig:ref_eg}
% \vspace{-0.2cm}
% \end{figure*}
% %%%%%%%%%%%%% figure %%%%%%%%%%%%%%%

To overcome this limitation, we propose a novel attention network, referred to as \textit{progressive attention network} (PAN), which enables precise attention over objects of different scales and shapes by attaching attentive mechanisms to multiple layers within a convolutional neural network (CNN).
More specifically, the proposed network predicts attentions on intermediate feature maps and forwards the attended feature maps in each layer to the subsequent layers in CNN.
%More specifically, the proposed network forces attention prediction in intermediate feature maps by forwarding the attended feature maps in each layer to the subsequent layers in the CNN.
%{\color{red}
% Such attention process enables precisely shaped attentions by progressively attending to multiple intermediate feature maps with different resolutions and aggregating these attentions through forward path of CNN.
% Since a feature to be attended in the current feature map is obtained by combining attended features in finer resolutions, the network can learn to distill the precise spatial support by observing local contexts during attention prediction.
%Since a feature to be attended in the current feature map is obtained by combining lower-level features with smaller receptive fields, the network can learn to distill the precise spatial support relevant to the target objects as final attention.
Moreover, we improve the proposed progressive attention by replacing feature aggregation, which may distort the original feature semantics, with hard attention via likelihood marginalization.
%}
The contribution of this work is four-fold:
\begin{itemize}\setlength\itemsep{-0.05cm}
\item A novel attention model (progressive attention network) learned to handle accurate scale and shape of attentions for a target object,
\item Integration of hard attention with likelihood marginalization into the proposed progressive attention networks,
\item Use of local contexts to improve stability of the progressive attention model,
\item Significant performance improvement over traditional single-step attention models in query-specific visual attribute prediction tasks.
\end{itemize}

The rest of this paper is organized as follows. 
%We first review related work and  the soft attention model in Section~\ref{relwork} and~\ref{satt}, respectively. 
We first review related work in Section~\ref{relwork}. 
Section~\ref{pan} describes the proposed model with local context information. 
We then present our experimental results on several datasets in Section~\ref{exp} and conclude the paper in Section~\ref{conclusion}.

==> BMVC 2018 Camera Ready/sections/progressive_attention_networks.tex <==
% !TEX root = ../main.tex

\setlength{\abovedisplayskip}{1pt}
\setlength{\belowdisplayskip}{1pt}

\vspace{-0.2cm}

\section{Progressive Attention Networks (PANs)}
\vspace{-0.1cm}
\label{pan}
To alleviate the limitations of existing attention models in handling variable object scales and shapes, we propose a progressive attention mechanism. 
We describe technical details about our attention model in this section.
\iffalse
In the proposed model, irrelevant features at different scales are suppressed by attention filtering steps in multiple CNN layers, and computation is focused on the remaining features corresponding to regions of interest.
%In this way, the network generates an attended feature map in each layer of CNN involving attentive process, and each attended feature map is then forwarded to the next layer of the CNN for construction of the following feature map, which is illustrated in Figure~\ref{fig:architecture}. 
In each attention layer, the model predicts an attention map given the input query and the current feature map via an attention module, and then the attention map is multiplied to the feature map in each channel to obtain an attended feature map.
In each layer, each attended feature map is then forwarded to the next layer of CNN for construction of the following feature map, which is illustrated in Figure~\ref{fig:architecture}. 
This progressive attention process allows us to estimate precise details of attention areas while maintaining deep representations appropriate for high-level inference tasks.
\fi


%
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\begin{figure*}[t]
\centering
\includegraphics[width=1\linewidth] {figures/architecture.pdf}
\vspace{-0.15cm}
\caption{Overall procedure of our progressive attention model.
Attentive processes are successively applied to feature maps at multiple layers and the resulting attended feature maps are used as input feature maps for the next convolution layers in the CNN.
Attention probabilities $\alpha^l$ are estimated from feature maps and input query.
In the last attention layer, (a) the attended feature maps are aggregated to a single feature vector (by sum pooling) as in soft attention and fed to the final attribute classifier, or (b) attention probabilities are used to marginalize attribute predictions from hard-selected feature at each spatial location as in hard attention.
The bar graphs in dotted cube denote attribute prediction results from individual spatial locations and $\Sigma$ in circle represents marginalization with attention probabilities.
}
\label{fig:architecture}
\vspace{-0.3cm}
\end{figure*}
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%

\vspace{-0.2cm}
\subsection{Progressive Attentive Process}

Let ${\bm{f}}^l \in \mathbb{R}^{H_l\times W_l\times C_l}$ be an output feature map of a layer $l \in \{0, \dots, L\}$ in CNN with width $W_l$, height $H_l$ and number of channels $C_l$, and $f^l_{i,j} \in \mathbb{R}^{C_l}$ be a feature at $(i, j)$ of feature map ${\bm{f}}^l$.
In the proposed model, an attentive process is applied to multiple layers of CNN and we obtain the following attended feature map ${\bm{\hat{f}}}^l = [ \hat{f}_{i,j}^l  ]$, where
%
\begin{equation}
\hat{f}^l_{i,j}=\alpha^l_{i,j} f^l_{i,j}.
\end{equation}
%
In the above equation, attention probability $\alpha^l_{i,j}$ for a feature $f^l_{i,j}$ and a query $q$ are given by
\begin{align}
s^l_{i, j} = g^l_\mathrm{att}(f^l_{i, j}, q; \bm{\theta}^l_\mathrm{att}), ~~~~~\text{and}~~~~~
% \end{align}
% and
% \begin{align}
\alpha_{i,j}^l = 
	\begin{cases}
		\mathrm{softmax}_{i,j}(\bm{s}^l) & \text{if} ~~ l=L \\
		\sigma(s_{i,j}^l) & \text{otherwise}
	\end{cases}
\label{eq:att}
\end{align}
where $g^l_\mathrm{att}(\cdot)$ denotes the attention function with a set of parameters $\bm{\theta}^l_\mathrm{att}$, $s^l_{i, j}$ is the attention score at $(i, j)$, and $\sigma(\cdot)$ is a sigmoid function.
The attention probability at each location is estimated independently in the same feature map; a sigmoid function is employed to constrain attention probabilities between 0 and 1. 
For the last layer of attention, we use a softmax function over the entire spatial region for later feature aggregation.

Unlike the soft attention model~\cite{showAtt}, the attended feature map ${\bm{\hat{f}}}^l$ in the intermediate attention layers is not summed up to generate a single vector representation of the attended regions.
Instead, the attended feature map is forwarded to the next layer as an input to compute the next feature map, which is given by
\begin{equation}
{\bm{f}}^{l+1} = g^{l+1}_\mathrm{CNN}(\bm{\hat{f}}^l; \bm{\theta}^{l+1}_\mathrm{CNN}) %= g^{l+1}_\mathrm{CNN}( {\bm r} (\bm{\alpha}^l , {C^l} ) \odot \bm{f}^l ; \bm{\theta}^{l+1}_\mathrm{CNN})
\label{eq:attended_feature_map_recursion}
\end{equation}
%where $g^{l+1}_\mathrm{CNN}(\cdot)$ is the next CNN operations parameterized by $\bm{\theta}^l_\mathrm{CNN}$, ${\bm r} (\bm{\alpha}^l , {C^l} )$ denotes $C^l$ times replication of $\bm{\alpha}^l$ in its channel direction, and $\odot$ denotes elementwise multiplication.
where $g^{l+1}_\mathrm{CNN}(\cdot)$ is the convolution operation at layer $l+1$ in CNN parameterized by $\bm{\theta}^{l+1}_\mathrm{CNN}$.%, ${\bm r} (\bm{\alpha}^l , {C^l} )$ denotes $C^l$ times replication of $\bm{\alpha}^l$ in its channel direction, and $\odot$ denotes elementwise multiplication.
%
This feedforward procedure with attentive processes in CNN is performed from the input layer, where ${\bm{f}}^{0} = I$, until ${\bm{\hat{f}}}^L$ is obtained.
The attended feature $f^\mathrm{att}$ is finally retrieved by summing up all the features in the final attended feature map ${\bm{\hat{f}}}^L$ as in soft attention, which is given by
\begin{equation}
f^\mathrm{att}= \sum_i^H{\sum_j^W{\hat{f}^L_{i,j}}}= \sum_i^H \sum_j^W \alpha^L_{i, j}f^L_{i, j}.
\label{eq:att_feat}
\end{equation}
The attended feature $f^\mathrm{att}$ obtained by this process is then used as the input to visual attribute classifier as shown in Figure~\ref{fig:architecture}a.

In our models, we place the attention layers to the output of max pooling layers instead of every layer in CNN because the reduction of feature resolution within CNN mainly comes from pooling layers.
In practice, we can also skip the first few pooling layers and attach the attention module only to the outputs of last $K$ pooling layers.
%If one uses a convolution layer with a stride larger than one, which downscales spatial dimension of a feature map, an attention layer may be placed after the convolution layer.

\vspace{-0.3cm}
\subsection{Incorporating Hard Attention}
\vspace{-0.1cm}
The derivation of the final attended feature $f^\mathrm{att}$ shown in Eq.~\eqref{eq:att_feat} is similar to soft attention mechanism.
However, since $f^\mathrm{att}$ is obtained by a weighted sum of features at all locations, it loses semantic layout of the original feature map. 
To overcome this limitation, we extend our model to incorporate hard attention.
Given the final feature map $\bm{f}^L$, the hard attention model predicts an answer distribution using the selected feature $f^L_{i,j}$ as
\begin{equation}
    p(a|\bm{f}^L, i, j) = H(f^L_{i,j})
\end{equation}
where $a$ is the predicted answer and $H(\cdot)$ is the visual attribute classifier.
The final answer distribution given the feature map $\bm{f}^L$ is obtained by
\begin{align}
%    p(a|\bm{f}^L) & = \sum_{i}^{H}\sum_{j}^{W}{p(a|\bm{f}^L, i, j)p(i, j|\bm{f}^L)} \nonumber \\
%                  & = \sum_{i}^{H}\sum_{j}^{W}{H(f^L_{i,j})\alpha^L_{i,j}}
    p(a|\bm{f}^L) = \sum_{i}^{H}\sum_{j}^{W}{p(a|\bm{f}^L, i, j)p(i, j|\bm{f}^L)} = \sum_{i}^{H}\sum_{j}^{W}{H(f^L_{i,j})\alpha^L_{i,j}}
\end{align}
where $p(i, j|\bm{f}^L)$ is modeled by $\alpha^L_{i,j}$ in Eq.~\eqref{eq:att}.
This marginalization eliminates the need for REINFORCE technique used in \cite{showAtt} by removing the hard selection process, and helps maintain the unique characteristics of feature maps.

\iffalse
In its original proposal from \cite{showAtt}, hard attention model hard-selects a single attention sequence for captioning since the search space for hard attention increases exponentially making it intractable to marginalize for every attention sequence.
However, in visual attribute prediction, the search space for single attention process is relatively small and thus it is feasible to marginalize the predictions from every location using the attention probabilities.
\fi

\vspace{-0.3cm}
\subsection{Multi-Resolution Attention Estimation}
\vspace{-0.1cm}
As shown in Eq.~\eqref{eq:att}, the resolution of attention probability map $\bm{\alpha}^l$ depends on the size of the feature map in the corresponding layer.
%Due to the nature of a CNN with convolution and pooling layers, the resolution of $\bm{\alpha}^l$ will decrease with increasing depth of the layer. 
Since the resolution of $\bm{\alpha}^l$ decreases inherently with increasing depth of CNNs and the attentive processes are performed over multiple layers recursively in our framework, we can attend to the regions with arbitrary resolutions even in higher layers.
Hence, the proposed network exploits high-level semantics in deep representations for inference without losing attention resolution. 

%Our attentive process is opposite to more intuitive coarse-to-fine approaches.
%However, the fine-to-coarse attention process in PAN is still very effective in predicting fine attention shapes as the attention information is aggregated over layers. 
The progressive attention model is also effective in predicting fine attention shapes as attention information is aggregated over multiple layers to suppress irrelevant structures at different levels. 
In lower layers, features whose receptive fields contain small distractors are suppressed first while the features from a part of large distractors remain intact.
In higher layers, features corresponding to these large distractors would have low attention probability as each feature contains information from larger receptive fields enabling the attention module to distinguish between distractors and target objects.
This phenomenon is demonstrated well in the qualitative results in our experiments (Section~\ref{exp}).
%
%However, what happens in our hierarchical attention network is similar in some sense to the coarse-to-fine methods because it learns to accumulate multi-resolution attention probability maps to identify the final attended regions.
%It forwards the high-resolution features corresponding to candidate regions of interest based on the observation of low-level features at the beginning, and then aggregates attention to the relevant regions of low-resolution (equivalently, filters out the irrelevant regions from low-resolution layer) based on high-level understanding later.
%We claim that a properly trained progressive attention network can estimate fine-grained attention probability maps through the multi-resolution attentive processing.
%To incorporate local context information in each layer, we observe neighborhood features to estimate attention probability map, which is critical for the effectiveness of the progressive attention process and %facilitate the training procedure.
%We will elaborate this technique in the next subsection.
An additional benefit of our progressive attention is that inference is based only on feedforward procedure.
%it is more straightforward during inference since it is a pure feedforward network.


%
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\includegraphics[width=0.6\linewidth] {figures/local_context.pdf}
\vspace{-0.2cm}
\caption{Attention estimation (a) without and (b) with local context. In (a), $\alpha^l_{i,j}$ is predicted from $f^l_{i,j}$ only while its spatially adjacent features are also employed to estimate $\alpha^l_{i,j}$ in (b).}
\label{fig:local_context}
\vspace{-0.5cm}
\end{figure}
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%


\vspace{-0.3cm}
\subsection{Local Context}
\vspace{-0.1cm}
%A basic version of PAN discussed so far predicts an attention probability $\alpha^l_{i,j}$ based solely on the feature $f^l_{i,j}$ at a single feature map location.
PAN can improve the quality of attention estimation by allowing its attention layers to observe a local context of the target feature.
%The use of local context makes it possible for the attention layer to further abstract the features.
%However, the attended feature $\hat{f}^l_{i,j}$ is supposed to refer to its neighborhood through convolution or pooling operations in the subsequent layers.
%This creates a gap between the attention process and the subsequent operations in CNN in terms of their capability of observable regions. 
%This gap could make the hierarchical attention network fail to identify regions of interest accurately and reduces the effectiveness in training our attention network. 
%
%We bridge this gap by allowing the attention network at each layer to observe a local context of the target feature during attention prediction. 
The local context $\mathcal{F}^l_{i, j}$ of a feature $f^l_{i,j}$ is composed of its spatially adjacent features as illustrated in Figure~\ref{fig:local_context}, and is formally denoted by $\mathcal{F}^l_{i,j}=\{f^l_{s,t} | i-\delta \le s \le i+\delta, j-\delta \le t \le j+\delta \}$.
%For example, the local context can be given by $\mathcal{F}^l_{i,j}=\{f^l_{s,t} | i-\delta \le s \le i+\delta, j-\delta \le t \le j+\delta \}$ as illustrated in Figure~\ref{fig:local_context}. 
The attention score is now predicted by the attention network with local context as
\begin{equation}
%s^l_{i, j} = g^l_{\mathrm{att}}(f^l_{i, j}, \mathcal{F}^l_{i, j}, q; \bm{\theta}^l_{\mathrm{att}}).
s^l_{i, j} = g^l_{\mathrm{att}}(\mathcal{F}^l_{i, j}, q; \bm{\theta}^l_{\mathrm{att}}).
\end{equation}
In our architecture, the area of the local context is given by the filter size corresponding to the composite operation of convolution followed by pooling in the next layer.
The local context does not need to be considered in the last layer of attention since its activations are used to compute the final attended feature map.
%Local context improves attention prediction as it enables the centroid feature to be compared with surrounding features, which makes the estimated attention more discriminative.
Local context improves attention prediction quality by comparing centroid features with their surroundings and making the estimated attention more discriminative.



\vspace{-0.3cm}
\subsection{Training Progressive Attention Networks}
\vspace{-0.1cm}

Training a PAN is as simple as training a soft attention network~\cite{showAtt} because every operation within the network is differentiable.
The entire network with both soft and hard attention is trained end-to-end by the standard backpropagation minimizing the cross entropy of the object-specific visual attributes.
%PAN incorporating hard attention is also fully differentiable, and training procedure is straightforward.
When we train it from a pretrained CNN, the CNN part should always be fine-tuned together since the intermediate attention maps may change the input distributions of their associated layers in the CNN.
%On the other hand, fine-tuning CNN is not required for the soft attention although it generally improves performance.

==> BMVC 2018 Camera Ready/sections/related_work.tex <==
% !TEX root = ../main.tex

\section{Related Work}
\label{relwork}

%
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%
\begin{figure}[t]
\centering
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/ref_eg/0.png}
\vspace{-0.15cm}
\subcaption{input image}
\end{subfigure}
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/ref_eg/1.png}
\vspace{-0.15cm}
\subcaption{first attention}
\end{subfigure}
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/ref_eg/2.png}
\vspace{-0.15cm}
\subcaption{second attention}
\end{subfigure}
\vspace{0.1cm}
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/ref_eg/3.png}
\vspace{-0.15cm}
\subcaption{third attention}
\end{subfigure}
\begin{subfigure}[b]{0.19\linewidth}
\centering
\includegraphics[width=0.8\textwidth]{figures/ref_eg/4.png}
\vspace{-0.15cm}
\subcaption{final attention}
\end{subfigure}
\vspace{-0.3cm}
\caption{
%An example reference problem (with query 7 and answer {\it{red}}) and intermediate attention maps using our progressive attention. 
Intermediate attention maps of our progressive attention method to solve a reference problem (with query 7 and answer {\it{red}}).
It shows that attention is gradually refined through the network layers for resolving the reference problem. Distracting patterns in smaller scales are suppressed at earlier layers while those in larger scales (\eg, 9) are suppressed at later layers with larger receptive fields.
All attended images are independently rescaled for better visualization.}
\label{fig:ref_eg}
\vspace{-0.5cm}
\end{figure}
%%%%%%%%%%%%% figure %%%%%%%%%%%%%%%

\paragraph{Attention on features}
The most straightforward attention mechanism is a feature based method, which selects a subset of features by explicitly attaching an attention model to NN architectures.
This approach has improved performance in many tasks~\cite{showAtt,stackAtt,compQA,askAtt,mtatt1,mtatt2,memNet,NTM}.
For example, it has been used to handle sequences of variable lengths in neural machine translation models~\cite{mtatt1,mtatt2}, speech recognition~\cite{attASR} and handwriting generation~\cite{firstAtt}, and manage memory access mechanisms for memory networks~\cite{memNet} and neural turing machines~\cite{NTM}.
%For example, they have been used to handle sequences of variable lengths in neural machine translation models~\citep{mtatt1,mtatt2} and manage memory access mechanisms for memory networks~\citep{memNet} and neural turing machines~\citep{NTM}. 
When applied to computer vision tasks to resolve reference problems, these models are designed to pay attention to CNN features corresponding to subregions in input images.
Image caption generation and visual question answering are often benefited from this attention mechanism~\cite{zheng2017learning,yu2017multi,showAtt,stackAtt,compQA,askAtt}.

%There have been several approaches iteratively performing attentive processes to resolve relations between targets.
%\cite{stackAtt} iteratively attend to images conditioned on the previous attention states for visual question answering as the objects of interest are often not specified explicitly in questions but implicitly in relational expressions about the target objects.
%Also, \cite{memNet} and \cite{NTM} incorporate attention mechanisms to memory cells iteratively to retrieve different values stored in the memory.
%Our proposed model is similar in spirit of iterative attention but aimed at attending to a single target object via operating on multiple CNN layers progressively, \ie attention information is predicted progressively from feature maps through multiple layers of CNN to capture the fine shapes of the target object.

\vspace{-0.3cm}
\paragraph{Attention by image transformation}
Another stream of attention model is image transformation.
This approach identifies transformation parameters fitting region of interest.
%These approaches transform a regular grid and sample from the input image with the transformed grid whose element corresponds to a location in the input image.
\cite{multiAtt}  and \cite{recurrentAtt} transform an input image with predicted translation parameters ($t_x$ and $t_y$) and a fixed scale factor ($\hat{s}<1$) for image classification or multiple object recognition. 
Scale factor is also predicted in \cite{draw} for image generation.
%where the network uses Gaussian filters for sampling. 
Spatial transformer networks (STNs) predict all six parameters of affine transformation, and even extend it to a projective transformation and a thin plate spline transformation~\cite{STN}. 
%Because all these transformations used in \cite{STN} involve scale factors, STNs are capable of dealing with objects in different sizes.
%However, STN is limited when there are multiple candidate regions for attention.
However, STN is limited to attending a single candidate region defined by a small number of parameters in an image.
Our model overcomes this issue by formulating attention as progressive filtering on feature maps instead of assuming that objects are roughly aligned by a constrained spatial transformation.
%We believe this is because the gradient signal gives only an indirect guide to the target object due to lack of supervision. 




\vspace{-0.3cm}
\paragraph{Multiple attention processes}
There have been several approaches iteratively performing attentive processes to utilize relations between objects.
For example, \cite{stackAtt} iteratively attends to images conditioned on the previous attention states for visual question answering.
%{\color{red}as the objects of interest are often not specified explicitly in questions but implicitly in relational expressions about target objects.}
Iterative attention mechanisms to memory cells is incorporated to retrieve different values stored in the memory~\cite{memNet,NTM}.
In \cite{STN}, an extension of STN to multiple transformer layers has also been presented but is still limited to rigid shape of attention.
Our model is similar to these approaches, but aims to attend to target regions via operating on multiple CNN layers in a progressive manner; attention information is predicted progressively from feature maps through multiple layers of CNN to capture the detailed shapes of target objects.

\iffalse
In \cite{STN}, the authors also conducted an experiment with a network with multiple transformer layers.
However, the attention shapes of STNs are still constrained to the predefined type of transformation regardless of the number of transformers.
In contrast, the proposed method improves the quality of attention shapes through progressive attention process.
\cite{dasNet} introduced a deep network, which manipulates intermediate features of a fixed classifier through channelwise attention process.
However, this method does not explore spatial attention process.
%Although the channel-wise attention process is used at multiple layers of the network to manipulate the intermediate feature representations, they did not explore spatial attention process.
More importantly, it requires to have an accurate pretrained classifier for the target classes prior to learning attention while pretraining a general query-specific attribute classifier is not trivial.
It is also notable that both \cite{STN} and \cite{dasNet} target simple classification tasks without queries while we aim to tackle the query-specific attribute prediction task, where answers for a single input image may vary depending on the input query.
\fi

\vspace{-0.3cm}
\paragraph{Training attention models}
%The soft attention model sums up features weighted by the attention probabilities.
The networks with soft attention are fully differentiable and thus trainable end-to-end by backpropagation.
Stochastic hard attention has been introduced in \cite{showAtt,reinforceNTM}, where networks explicitly select a single feature location based on the predicted attention probability map.
%Because the explicit selection (or sampling) procedure is not differentiable, additional techniques, such as variational lower bound and Monte Carlo method resulting in the REINFORCE learning rule~\cite{reinforce}, were used to make networks trainable with a large search space defined by latent variables.
Because the explicit selection (or sampling) procedure is not differentiable, hard attention methods employ REINFORCE learning rule~\cite{reinforce} for training.
%Even though this hard attention model performed slightly better than soft attention on image caption generation, the size of the attended region is still fixed and even more restricted in shape than a soft attention model.
Transformation-based attention models~\cite{multiAtt,recurrentAtt} are typically learned by REINFORCE as well while STN~\cite{STN} proposes a fully differentiable formulation suitable for end-to-end learning.
%This formulation can also be applied to the other transformation based attention methods for facilitating training. 
%Compared to these attention networks, 
The proposed network has advantage of end-to-end trainability by a standard backpropagation without any extra technique. %since every operation within the network is differentiable.
